Constraining Accretion Regimes of Little Red Dots from Their Variability

The ``little red dots'' (LRDs) are photometrically and spectroscopically non-variable on rest-frame baselines of months, with a $5.9\sigma$ deficit relative to ordinary active galactic nuclei (AGNs). If we consider LRDs to be accreting black holes, this non-varying could be a clue about the nature of the accretion. Here, we present a general semi-analytic model of variability from super-Eddington (slim) accretion disks. We consider three mechanisms that play crucial roles in the observed variability, viz., advective attenuation, photospheric averaging, and photon diffusion filter. With this, above $\mdot \sim$ a few, the fractional rms collapses steeply with $\mdot$. Comparing with JWST monitoring constraints, we find that the non-detection of LRD variability requires $\mdot \gtrsim 30$ for $M_{\rm BH}\sim10^{7}\,M_\odot$ on a 0.5\,yr rest-frame baseline; a Monte Carlo forward model of the TWINKLE non-detections of 18 LRDs sharpens this to $\mdot\gtrsim60$ at 95\% confidence. On current baselines, these non-detections remain formally degenerate with a frozen sub-Eddington disk ($\mdot\lesssim0.1$). Longer monitoring will separate the two regimes as the frozen-disk variability grows with baseline, while the super-Eddington collapse does not. The same framework predicts strongly suppressed X-ray variability, testable with future X-ray observatories.

==> ms-02 <==
\begin{thebibliography}{}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi
\providecommand{\url}[1]{\href{#1}{#1}}
\providecommand{\dodoi}[1]{doi:~\href{http://doi.org/#1}{\nolinkurl{#1}}}
\providecommand{\doeprint}[1]{\href{http://ascl.net/#1}{\nolinkurl{http://ascl.net/#1}}}
\providecommand{\doarXiv}[1]{\href{https://arxiv.org/abs/#1}{\nolinkurl{https://arxiv.org/abs/#1}}}

% type= article
\bibitem[{M.~A. {Abramowicz} {et~al.}(1988){Abramowicz}, {Czerny}, {Lasota}, \& {Szuszkiewicz}}]{abramowicz88}
{Abramowicz}, M.~A., {Czerny}, B., {Lasota}, J.~P., \& {Szuszkiewicz}, E. 1988, \bibinfo{title}{{Slim Accretion Disks},} \apj, 332, 646, \dodoi{10.1086/166683}

% type= article
\bibitem[{Y.~L. {Ai} {et~al.}(2010){Ai}, {Yuan}, {Zhou}, {Wang}, {Dong}, {Wang}, \& {Lu}}]{ai10}
{Ai}, Y.~L., {Yuan}, W., {Zhou}, H.~Y., {et~al.} 2010, \bibinfo{title}{{Dependence of the Optical/Ultraviolet Variability on the Emission-line Properties and Eddington Ratio in Active Galactic Nuclei},} \apjl, 716, L31, \dodoi{10.1088/2041-8205/716/1/L31}

% type= article
\bibitem[{H.~B. {Akins} {et~al.}(2025){Akins}, {Casey}, {Lambrides}, {Allen}, {Andika}, {Brinch}, {Champagne}, {Cooper}, {Ding}, {Drakos}, {Faisst}, {Finkelstein}, {Franco}, {Fujimoto}, {Gentile}, {Gillman}, {Gozaliasl}, {Harish}, {Hayward}, {Hirschmann}, {Ilbert}, {Kartaltepe}, {Kocevski}, {Koekemoer}, {Kokorev}, {Liu}, {Long}, {McCracken}, {McKinney}, {Onoue}, {Paquereau}, {Renzini}, {Rhodes}, {Robertson}, {Shuntov}, {Silverman}, {Tanaka}, {Toft}, {Trakhtenbrot}, {Valentino}, \& {Zavala}}]{akins25}
{Akins}, H.~B., {Casey}, C.~M., {Lambrides}, E., {et~al.} 2025, \bibinfo{title}{{COSMOS-Web: The Overabundance and Physical Nature of ``Little Red Dots''{\textemdash}Implications for Early Galaxy and SMBH Assembly},} \apj, 991, 37, \dodoi{10.3847/1538-4357/ade984}

% type= article
\bibitem[{T.~T. {Ananna} {et~al.}(2024){Ananna}, {Bogd{\'a}n}, {Kov{\'a}cs}, {Natarajan}, \& {Hickox}}]{ananna24}
{Ananna}, T.~T., {Bogd{\'a}n}, {\'A}., {Kov{\'a}cs}, O.~E., {Natarajan}, P., \& {Hickox}, R.~C. 2024, \bibinfo{title}{{X-Ray View of Little Red Dots: Do They Host Supermassive Black Holes?},} \apjl, 969, L18, \dodoi{10.3847/2041-8213/ad5669}

% type= article
\bibitem[{P. {Ar{\'e}valo} \& P. {Uttley}(2006){Ar{\'e}valo} \& {Uttley}}]{arevalo06}
{Ar{\'e}valo}, P., \& {Uttley}, P. 2006, \bibinfo{title}{{Investigating a fluctuating-accretion model for the spectral-timing properties of accreting black hole systems},} \mnras, 367, 801, \dodoi{10.1111/j.1365-2966.2006.09989.x}

% type= article
\bibitem[{C.~J. {Burke} {et~al.}(2021){Burke}, {Shen}, {Blaes}, {Gammie}, {Horne}, {Jiang}, {Liu}, {McHardy}, {Morgan}, {Scaringi}, \& {Yang}}]{burke21}
{Burke}, C.~J., {Shen}, Y., {Blaes}, O., {et~al.} 2021, \bibinfo{title}{{A characteristic optical variability time scale in astrophysical accretion disks},} Science, 373, 789, \dodoi{10.1126/science.abg9933}

% type= article
\bibitem[{M. {Cantiello} {et~al.}(2026){Cantiello}, {Hassan}, {Perna}, {Armitage}, {Begelman}, {Jiang}, {Ryu}, \& {Townsend}}]{cantiello25}
{Cantiello}, M., {Hassan}, J.~B., {Perna}, R., {et~al.} 2026, \bibinfo{title}{{Pulsational Instability of Quasi-stars: Interpreting the Variability of Little Red Dots},} \apjl, 1000, L4, \dodoi{10.3847/2041-8213/ae4729}

% type= article
\bibitem[{C.~M. {Casey} {et~al.}(2024){Casey}, {Akins}, {Kokorev}, {McKinney}, {Cooper}, {Long}, {Franco}, \& {Manning}}]{casey24}
{Casey}, C.~M., {Akins}, H.~B., {Kokorev}, V., {et~al.} 2024, \bibinfo{title}{{Dust in Little Red Dots},} \apjl, 975, L4, \dodoi{10.3847/2041-8213/ad7ba7}

% type= article
\bibitem[{A. {de Graaff} {et~al.}(2025){de Graaff}, {Rix}, {Naidu}, {Labb{\'e}}, {Wang}, {Leja}, {Matthee}, {Katz}, {Greene}, {Hviding}, \& et~al.}]{degraaf25}
{de Graaff}, A., {Rix}, H.-W., {Naidu}, R.~P., {et~al.} 2025, \bibinfo{title}{{A remarkable ruby: Absorption in dense gas, rather than evolved stars, drives the extreme Balmer break of a little red dot at z = 3.5},} \aap, 701, A168, \dodoi{10.1051/0004-6361/202554681}

% type= article
\bibitem[{I. {Delvecchio} {et~al.}(2025){Delvecchio}, {Daddi}, {Magnelli}, {Elbaz}, {Giavalisco}, {Traina}, {Lanzuisi}, {Akins}, {Belli}, {Casey}, \& et~al.}]{Delvecchio2025}
{Delvecchio}, I., {Daddi}, E., {Magnelli}, B., {et~al.} 2025, \bibinfo{title}{{Active galactic nuclei-heated dust revealed in ``little red dots''},} \aap, 704, A313, \dodoi{10.1051/0004-6361/202557164}

% type= article
\bibitem[{S. {Gezari}(2021){Gezari}}]{gezari21}
{Gezari}, S. 2021, \bibinfo{title}{{Tidal Disruption Events},} \araa, 59, 21, \dodoi{10.1146/annurev-astro-111720-030029}

% type= article
\bibitem[{J.~E. {Greene} {et~al.}(2024){Greene}, {Labbe}, {Goulding}, {Furtak}, {Chemerynska}, {Kokorev}, {Dayal}, {Volonteri}, {Williams}, {Wang}, {Setton}, {Burgasser}, {Bezanson}, {Atek}, {Brammer}, {Cutler}, {Feldmann}, {Fujimoto}, {Glazebrook}, {de Graaff}, {Khullar}, {Leja}, {Marchesini}, {Maseda}, {Matthee}, {Miller}, {Naidu}, {Nanayakkara}, {Oesch}, {Pan}, {Papovich}, {Price}, {van Dokkum}, {Weaver}, {Whitaker}, \& {Zitrin}}]{greene24}
{Greene}, J.~E., {Labbe}, I., {Goulding}, A.~D., {et~al.} 2024, \bibinfo{title}{{UNCOVER Spectroscopy Confirms the Surprising Ubiquity of Active Galactic Nuclei in Red Sources at z > 5},} \apj, 964, 39, \dodoi{10.3847/1538-4357/ad1e5f}

% type= article
\bibitem[{J.~E. {Greene} {et~al.}(2026){Greene}, {Setton}, {Furtak}, {Naidu}, {Volonteri}, {Dayal}, {Labbe}, {van Dokkum}, {Bezanson}, {Brammer}, \& et~al.}]{Greene2026}
{Greene}, J.~E., {Setton}, D.~J., {Furtak}, L.~J., {et~al.} 2026, \bibinfo{title}{{What You See Is What You Get: Empirically Measured Bolometric Luminosities of Little Red Dots},} \apj, 996, 129, \dodoi{10.3847/1538-4357/ae1836}

% type= article
\bibitem[{Y. {Harikane} {et~al.}(2023){Harikane}, {Zhang}, {Nakajima}, {Ouchi}, {Isobe}, {Ono}, {Hatano}, {Xu}, \& {Umeda}}]{harikane23}
{Harikane}, Y., {Zhang}, Y., {Nakajima}, K., {et~al.} 2023, \bibinfo{title}{{A JWST/NIRSpec First Census of Broad-line AGNs at z = 4-7: Detection of 10 Faint AGNs with M $_{BH}$ {}10$^{6}$-{}10$^{8}$ M $_{☉}$ and Their Host Galaxy Properties},} \apj, 959, 39, \dodoi{10.3847/1538-4357/ad029e}

% type= article
\bibitem[{L.~C. {Ho}(2008){Ho}}]{ho08}
{Ho}, L.~C. 2008, \bibinfo{title}{{Nuclear activity in nearby galaxies.},} \araa, 46, 475, \dodoi{10.1146/annurev.astro.45.051806.110546}

% type= article
\bibitem[{K. {Inayoshi}(2025){Inayoshi}}]{inayoshi25a}
{Inayoshi}, K. 2025, \bibinfo{title}{{Little Red Dots as the Very First Activity of Black Hole Growth},} \apjl, 988, L22, \dodoi{10.3847/2041-8213/adea66}

% type= article
\bibitem[{K. {Inayoshi} {et~al.}(2025){Inayoshi}, {Kimura}, \& {Noda}}]{inayoshi25c}
{Inayoshi}, K., {Kimura}, S.~S., \& {Noda}, H. 2025, \bibinfo{title}{{Weakness of X-rays and variability in high-redshift active galactic nuclei with super-Eddington accretion},} \pasj, 77, 811, \dodoi{10.1093/pasj/psaf050}

% type= article
\bibitem[{K. {Inayoshi} \& R. {Maiolino}(2025){Inayoshi} \& {Maiolino}}]{inayoshi25b}
{Inayoshi}, K., \& {Maiolino}, R. 2025, \bibinfo{title}{{Extremely Dense Gas around Little Red Dots and High-redshift Active Galactic Nuclei: A Nonstellar Origin of the Balmer Break and Absorption Features},} \apjl, 980, L27, \dodoi{10.3847/2041-8213/adaebd}

% type= article
\bibitem[{Y.-F. {Jiang} {et~al.}(2019){Jiang}, {Stone}, \& {Davis}}]{jiang19}
{Jiang}, Y.-F., {Stone}, J.~M., \& {Davis}, S.~W. 2019, \bibinfo{title}{{Super-Eddington Accretion Disks around Supermassive Black Holes},} \apj, 880, 67, \dodoi{10.3847/1538-4357/ab29ff}

% type= article
\bibitem[{B.~C. {Kelly} {et~al.}(2009){Kelly}, {Bechtold}, \& {Siemiginowska}}]{kelly09}
{Kelly}, B.~C., {Bechtold}, J., \& {Siemiginowska}, A. 2009, \bibinfo{title}{{Are the Variations in Quasar Optical Flux Driven by Thermal Fluctuations?},} \apj, 698, 895, \dodoi{10.1088/0004-637X/698/1/895}

% type= article
\bibitem[{B.~C. {Kelly} {et~al.}(2011){Kelly}, {Sobolewska}, \& {Siemiginowska}}]{Kelly11}
{Kelly}, B.~C., {Sobolewska}, M., \& {Siemiginowska}, A. 2011, \bibinfo{title}{{A Stochastic Model for the Luminosity Fluctuations of Accreting Black Holes},} \apj, 730, 52, \dodoi{10.1088/0004-637X/730/1/52}

% type= article
\bibitem[{D.~D. {Kocevski} {et~al.}(2023){Kocevski}, {Onoue}, {Inayoshi}, {Trump}, {Arrabal Haro}, {Grazian}, {Dickinson}, {Finkelstein}, {Kartaltepe}, {Hirschmann}, {Aird}, {Holwerda}, {Fujimoto}, {Juneau}, {Amor{\'\i}n}, {Backhaus}, {Bagley}, {Barro}, {Bell}, {Bisigello}, {Calabr{\`o}}, {Cleri}, {Cooper}, {Ding}, {Grogin}, {Ho}, {Hutchison}, {Inoue}, {Jiang}, {Jones}, {Koekemoer}, {Li}, {Li}, {McGrath}, {Molina}, {Papovich}, {P{\'e}rez-Gonz{\'a}lez}, {Pirzkal}, {Wilkins}, {Yang}, \& {Yung}}]{kocevski23}
{Kocevski}, D.~D., {Onoue}, M., {Inayoshi}, K., {et~al.} 2023, \bibinfo{title}{{Hidden Little Monsters: Spectroscopic Identification of Low-mass, Broad-line AGNs at z > 5 with CEERS},} \apjl, 954, L4, \dodoi{10.3847/2041-8213/ace5a0}

% type= article
\bibitem[{D.~D. {Kocevski} {et~al.}(2025){Kocevski}, {Finkelstein}, {Barro}, {Taylor}, {Calabr{\`o}}, {Laloux}, {Buchner}, {Trump}, {Leung}, {Yang}, {Dickinson}, {P{\'e}rez-Gonz{\'a}lez}, {Pacucci}, {Inayoshi}, {Somerville}, {McGrath}, {Akins}, {Bagley}, {Bowler}, {Bisigello}, {Carnall}, {Casey}, {Cheng}, {Cleri}, {Costantin}, {Cullen}, {Davis}, {Donnan}, {Dunlop}, {Ellis}, {Ferguson}, {Fujimoto}, {Fontana}, {Giavalisco}, {Grazian}, {Grogin}, {Hathi}, {Hirschmann}, {Huertas-Company}, {Holwerda}, {Illingworth}, {Juneau}, {Kartaltepe}, {Koekemoer}, {Li}, {Lucas}, {Magee}, {Mason}, {McLeod}, {McLure}, {Napolitano}, {Papovich}, {Pirzkal}, {Rodighiero}, {Santini}, {Wilkins}, \& {Yung}}]{kocevski25}
{Kocevski}, D.~D., {Finkelstein}, S.~L., {Barro}, G., {et~al.} 2025, \bibinfo{title}{{The Rise of Faint, Red Active Galactic Nuclei at z > 4: A Sample of Little Red Dots in the JWST Extragalactic Legacy Fields},} \apj, 986, 126, \dodoi{10.3847/1538-4357/adbc7d}

% type= article
\bibitem[{M. {Kokubo} \& Y. {Harikane}(2025){Kokubo} \& {Harikane}}]{kokubo25}
{Kokubo}, M., \& {Harikane}, Y. 2025, \bibinfo{title}{{Challenging the Active Galactic Nucleus Scenario for JWST/NIRSpec Little Red Dot and Non─Little Red Dot Broad H{\ensuremath{\alpha}} Emitters in Light of Nondetection of NIRCam Photometric Variability and X-Ray},} \apj, 995, 24, \dodoi{10.3847/1538-4357/ae119e}

% type= article
\bibitem[{I. {Labb{\'e}} {et~al.}(2023){Labb{\'e}}, {van Dokkum}, {Nelson}, {Bezanson}, {Suess}, {Leja}, {Brammer}, {Whitaker}, {Mathews}, {Stefanon}, \& {Wang}}]{labbe23}
{Labb{\'e}}, I., {van Dokkum}, P., {Nelson}, E., {et~al.} 2023, \bibinfo{title}{{A population of red candidate massive galaxies 600 Myr after the Big Bang},} \nat, 616, 266, \dodoi{10.1038/s41586-023-05786-2}

% type= article
\bibitem[{I. {Labbe} {et~al.}(2025){Labbe}, {Greene}, {Bezanson}, {Fujimoto}, {Furtak}, {Goulding}, {Matthee}, {Naidu}, {Oesch}, {Atek}, {Brammer}, {Chemerynska}, {Coe}, {Cutler}, {Dayal}, {Feldmann}, {Franx}, {Glazebrook}, {Leja}, {Maseda}, {Marchesini}, {Nanayakkara}, {Nelson}, {Pan}, {Papovich}, {Price}, {Suess}, {Wang}, {Weaver}, {Whitaker}, {Williams}, \& {Zitrin}}]{labbe25}
{Labbe}, I., {Greene}, J.~E., {Bezanson}, R., {et~al.} 2025, \bibinfo{title}{{UNCOVER: Candidate Red Active Galactic Nuclei at 3 < z < 7 with JWST and ALMA},} \apj, 978, 92, \dodoi{10.3847/1538-4357/ad3551}

% type= article
\bibitem[{R. {Lin} {et~al.}(2025){Lin}, {Zheng}, {Jiang}, {Yuan}, {Ho}, {Wang}, {Jiang}, {Rhoads}, {Malhotra}, {Barrientos}, \& et~al.}]{lin25}
{Lin}, R., {Zheng}, Z.-Y., {Jiang}, C., {et~al.} 2025, \bibinfo{title}{{Discovery of Local Analogs to JWST's Little Red Dots},} \apjl, 980, L34, \dodoi{10.3847/2041-8213/adaaf1}

% type= article
\bibitem[{R. {Lin} {et~al.}(2026){Lin}, {Zheng}, {Wang}, {Ho}, {Zavala}, {Zhang}, {Jiang}, {Lin}, {Yuan}, {Jiang}, \& et~al.}]{Lin26}
{Lin}, R., {Zheng}, Z.-Y., {Wang}, J., {et~al.} 2026, \bibinfo{title}{{Local Analogs of Little Red Dots: Optical Variability and Evidence for an Active Galactic Nucleus Origin},} \apj, 1005, 150, \dodoi{10.3847/1538-4357/ae74c6}

% type= misc
\bibitem[{Z. {Liu} {et~al.}(2026){Liu}, {Naidu}, {Secunda}, {Greene}, {Matthee}, {Chisholm}, {de Graaff}, {Robbins}, {Antwi-Danso}, {Brammer}, {Sun}, {Eilers}, {Fujimoto}, {Furtak}, {Kara}, {Kokorev}, {Marchesini}, {Oesch}, {Pierel}, {Shen}, {Simcoe}, {Torralba}, \& {Vogelsberger}}]{liu26}
{Liu}, Z., {Naidu}, R.~P., {Secunda}, A., {et~al.} 2026, {How I Wonder What You Are -- JWST's Little Red Dots do not TWINKLE}, \dodoi{10.48550/arXiv.2604.13000}

% type= article
\bibitem[{K.-X. {Lu} {et~al.}(2019){Lu}, {Huang}, {Zhang}, {Wang}, {Du}, {Hu}, {Xiao}, {Li}, {Bai}, {Bian}, {Yuan}, {Ho}, {Wang}, \& {SEAMBH Collaboration}}]{lu19}
{Lu}, K.-X., {Huang}, Y.-K., {Zhang}, Z.-X., {et~al.} 2019, \bibinfo{title}{{Supermassive Black Holes with High Accretion Rates in Active Galactic Nuclei. X. Optical Variability Characteristics},} \apj, 877, 23, \dodoi{10.3847/1538-4357/ab16e8}

% type= article
\bibitem[{Y.~E. {Lyubarskii}(1997){Lyubarskii}}]{lyubarskii97}
{Lyubarskii}, Y.~E. 1997, \bibinfo{title}{{Flicker noise in accretion discs},} \mnras, 292, 679, \dodoi{10.1093/mnras/292.3.679}

% type= article
\bibitem[{C.~L. {MacLeod} {et~al.}(2010){MacLeod}, {Ivezi{\'c}}, {Kochanek}, {Koz{\l}owski}, {Kelly}, {Bullock}, {Kimball}, {Sesar}, {Westman}, {Brooks}, {Gibson}, {Becker}, \& {de Vries}}]{macleod10}
{MacLeod}, C.~L., {Ivezi{\'c}}, {\v{Z}}., {Kochanek}, C.~S., {et~al.} 2010, \bibinfo{title}{{Modeling the Time Variability of SDSS Stripe 82 Quasars as a Damped Random Walk},} \apj, 721, 1014, \dodoi{10.1088/0004-637X/721/2/1014}

% type= misc
\bibitem[{P. {Madau} \& R. {Maiolino}(2026){Madau} \& {Maiolino}}]{madau26}
{Madau}, P., \& {Maiolino}, R. 2026, {Little Red Dots as Obscured Little Blue Dots: A Super-Eddington Unification Model}, \dodoi{10.48550/arXiv.2602.22386}

% type= article
\bibitem[{J. {Matthee} {et~al.}(2024){Matthee}, {Naidu}, {Brammer}, {Chisholm}, {Eilers}, {Goulding}, {Greene}, {Kashino}, {Labbe}, {Lilly}, {Mackenzie}, {Oesch}, {Weibel}, {Wuyts}, {Xiao}, {Bordoloi}, {Bouwens}, {van Dokkum}, {Illingworth}, {Kramarenko}, {Maseda}, {Mason}, {Meyer}, {Nelson}, {Reddy}, {Shivaei}, {Simcoe}, \& {Yue}}]{matthee24}
{Matthee}, J., {Naidu}, R.~P., {Brammer}, G., {et~al.} 2024, \bibinfo{title}{{Little Red Dots: An Abundant Population of Faint Active Galactic Nuclei at z {\ensuremath{\sim}} 5 Revealed by the EIGER and FRESCO JWST Surveys},} \apj, 963, 129, \dodoi{10.3847/1538-4357/ad2345}

% type= article
\bibitem[{R.~P. {Naidu} {et~al.}(2026){Naidu}, {Matthee}, {Katz}, {de Graaff}, {Oesch}, {Smith}, {Greene}, {Brammer}, {Weibel}, {Hviding}, {Chisholm}, {Labb{\'e}}, {Simcoe}, {Witten}, {Sun}, {Atek}, {Baggen}, {Belli}, {Bezanson}, {Boogaard}, {Bose}, {Bouwens}, {Covelo-Paz}, {Dayal}, {Fudamoto}, {Furtak}, {Giovinazzo}, {Goulding}, {Gronke}, {Heintz}, {Hirschmann}, {Illingworth}, {Inoue}, {Johnson}, {Leja}, {Leonova}, {McConachie}, {Maseda}, {Natarajan}, {Nelson}, {Setton}, {Shivaei}, {Sobral}, {Stefanon}, {Tacchella}, {Toft}, {Torralba}, {van Dokkum}, {van der Wel}, {Volonteri}, {Walter}, {Wang}, {Watson}, \& {Whitaker}}]{naidu25}
{Naidu}, R.~P., {Matthee}, J., {Katz}, H., {et~al.} 2026, \bibinfo{title}{{A gas-enshrouded and gas-reddened black hole at cosmic dawn},} \nat, 656, 329, \dodoi{10.1038/s41586-026-10846-4}

% type= article
\bibitem[{R. Narayan \& I. Yi(1994)Narayan \& Yi}]{Narayan1994Advection-dominatedSolution}
Narayan, R., \& Yi, I. 1994, \bibinfo{title}{{Advection-dominated Accretion: A Self-similar Solution},} 428, L13, \dodoi{10.1086/187381}

% type= article
\bibitem[{X.-W. {Ning} {et~al.}(2026){Ning}, {Hu}, {Yuan}, {Tang}, {Ma}, {Gua}, {Huang}, \& {Bian}}]{ning26}
{Ning}, X.-W., {Hu}, W.-J., {Yuan}, Z.-H., {et~al.} 2026, \bibinfo{title}{{Probing the Optical/UV Continuum Variability of Active Galactic Nuclei with the Damped Random Walk Model},} arXiv e-prints, arXiv:2610.27806, \dodoi{10.48550/arXiv.2610.27806}

% type= article
\bibitem[{K. {Ohsuga} {et~al.}(2005){Ohsuga}, {Mori}, {Nakamoto}, \& {Mineshige}}]{ohsuga05}
{Ohsuga}, K., {Mori}, M., {Nakamoto}, T., \& {Mineshige}, S. 2005, \bibinfo{title}{{Supercritical Accretion Flows around Black Holes: Two-dimensional, Radiation Pressure-dominated Disks with Photon Trapping},} \apj, 628, 368, \dodoi{10.1086/430728}

% type= article
\bibitem[{M. {Onoue} {et~al.}(2023){Onoue}, {Inayoshi}, {Ding}, {Li}, {Li}, {Molina}, {Inoue}, {Jiang}, \& {Ho}}]{onoue23}
{Onoue}, M., {Inayoshi}, K., {Ding}, X., {et~al.} 2023, \bibinfo{title}{{A Candidate for the Least-massive Black Hole in the First 1.1 Billion Years of the Universe},} \apjl, 942, L17, \dodoi{10.3847/2041-8213/aca9d3}

% type= article
\bibitem[{J. {Poutanen} {et~al.}(2007){Poutanen}, {Lipunova}, {Fabrika}, {Butkevich}, \& {Abolmasov}}]{poutanen07}
{Poutanen}, J., {Lipunova}, G., {Fabrika}, S., {Butkevich}, A.~G., \& {Abolmasov}, P. 2007, \bibinfo{title}{{Supercritically accreting stellar mass black holes as ultraluminous X-ray sources},} \mnras, 377, 1187, \dodoi{10.1111/j.1365-2966.2007.11668.x}

% type= article
\bibitem[{S. {Rakshit} \& C.~S. {Stalin}(2017){Rakshit} \& {Stalin}}]{rakshit17}
{Rakshit}, S., \& {Stalin}, C.~S. 2017, \bibinfo{title}{{Optical Variability of Narrow-line and Broad-line Seyfert 1 Galaxies},} \apj, 842, 96, \dodoi{10.3847/1538-4357/aa72f4}

% type= article
\bibitem[{A. {Sacchi} \& {\'A}. {Bogd{\'a}n}(2025){Sacchi} \& {Bogd{\'a}n}}]{Sacchi25}
{Sacchi}, A., \& {Bogd{\'a}n}, {\'A}. 2025, \bibinfo{title}{{Chandra Rules Out Super-Eddington Accretion Models for Little Red Dots},} \apjl, 989, L30, \dodoi{10.3847/2041-8213/adf5c8}

% type= article
\bibitem[{A. {Sadowski} \& R. {Narayan}(2016){Sadowski} \& {Narayan}}]{sadowski16}
{Sadowski}, A., \& {Narayan}, R. 2016, \bibinfo{title}{{Three-dimensional simulations of supercritical black hole accretion discs - luminosities, photon trapping and variability},} \mnras, 456, 3929, \dodoi{10.1093/mnras/stv2941}

% type= article
\bibitem[{A. {Secunda} {et~al.}(2026){Secunda}, {Somerville}, {Jiang}, {Greene}, {Furtak}, \& {Zitrin}}]{secunda26}
{Secunda}, A., {Somerville}, R.~S., {Jiang}, Y.-F., {et~al.} 2026, \bibinfo{title}{{Do Little Red Dots Vary?},} \apj, 996, 6, \dodoi{10.3847/1538-4357/ae1f08}

% type= article
\bibitem[{N.~I. {Shakura} \& R.~A. {Sunyaev}(1973){Shakura} \& {Sunyaev}}]{ss73}
{Shakura}, N.~I., \& {Sunyaev}, R.~A. 1973, \bibinfo{title}{{Black holes in binary systems. Observational appearance.},} \aap, 24, 337

% type= article
\bibitem[{W.~L. {Tee} {et~al.}(2025){Tee}, {Fan}, {Wang}, \& {Yang}}]{tee25}
{Tee}, W.~L., {Fan}, X., {Wang}, F., \& {Yang}, J. 2025, \bibinfo{title}{{Lack of Rest-frame Ultraviolet Variability in Little Red Dots Based on HST and JWST Observations},} \apjl, 983, L26, \dodoi{10.3847/2041-8213/adc5e3}

% type= article
\bibitem[{H.-T. {Wang} {et~al.}(2022){Wang}, {Su}, {Ge}, {Chen}, \& {Yu}}]{wang22}
{Wang}, H.-T., {Su}, Y.-P., {Ge}, X., {Chen}, Y.-Y., \& {Yu}, X.-L. 2022, \bibinfo{title}{{The Variability of the Narrow-line Seyfert 1 Galaxies from the Pan-STARRS's View},} Research in Astronomy and Astrophysics, 22, 015014, \dodoi{10.1088/1674-4527/ac3895}

% type= article
\bibitem[{K.-y. {Watarai} \& J. {Fukue}(1999){Watarai} \& {Fukue}}]{watarai99}
{Watarai}, K.-y., \& {Fukue}, J. 1999, \bibinfo{title}{{Radiative Disk Winds from a Self-Similar Slim Disk},} \pasj, 51, 725, \dodoi{10.1093/pasj/51.5.725}

% type= article
\bibitem[{B.~C. {Wilhite} {et~al.}(2008){Wilhite}, {Brunner}, {Grier}, {Schneider}, \& {vanden Berk}}]{wilhite08}
{Wilhite}, B.~C., {Brunner}, R.~J., {Grier}, C.~J., {Schneider}, D.~P., \& {vanden Berk}, D.~E. 2008, \bibinfo{title}{{On the variability of quasars: a link between the Eddington ratio and optical variability?},} \mnras, 383, 1232, \dodoi{10.1111/j.1365-2966.2007.12655.x}

% type= article
\bibitem[{F. {Yuan} \& R. {Narayan}(2014){Yuan} \& {Narayan}}]{yuan14}
{Yuan}, F., \& {Narayan}, R. 2014, \bibinfo{title}{{Hot Accretion Flows Around Black Holes},} \araa, 52, 529, \dodoi{10.1146/annurev-astro-082812-141003}

% type= article
\bibitem[{Z. {Zhang} {et~al.}(2025){Zhang}, {Jiang}, {Liu}, \& {Ho}}]{zhang25}
{Zhang}, Z., {Jiang}, L., {Liu}, W., \& {Ho}, L.~C. 2025, \bibinfo{title}{{Analysis of Multi-epoch JWST Images of {\ensuremath{\sim}}300 Little Red Dots: Tentative Detection of Variability in a Minority of Sources},} \apj, 985, 119, \dodoi{10.3847/1538-4357/adcb3e}

% type= article
\bibitem[{S. {Zhou} {et~al.}(2025){Zhou}, {Sun}, {Zhang}, {Chen}, \& {Ho}}]{Zhou-etal2025}
{Zhou}, S., {Sun}, M., {Zhang}, Z., {Chen}, J., \& {Ho}, L.~C. 2025, \bibinfo{title}{{On the Variability Features of Active Galactic Nuclei in Little Red Dots},} \apj, 991, 137, \dodoi{10.3847/1538-4357/adfd5f}

\end{thebibliography}

